Hands-Free One-Time and Continuous Authentication Using Glass Wearable Devices

Users with limited use of their hands, such as people suffering from disabilities of the arm, shoulder, and hand (DASH), face challenges when authenticating with computer terminals, specially with publicly accessible terminals such as ATMs. A new glass wearable device was recently introduced by Google and it was immediately welcomed by groups of users, such as the ones described above, as Google Glass allows them to perform actions, like taking a photo, using only verbal commands. This paper investigates whether glass wearable devices can be used to authenticate users, both to grant access (one-time) and to maintain access (continuous), in similar hands-free fashion. We do so by designing and implementing Gauth, a system that enables users to authenticate with a service simply by issuing a voice command, while facing the computer terminal they are going to use to access the service. To achieve this goal, we create a physical communication channel from the terminal to the device using machine readable visual codes, like QR codes, and utilize the device's network adapter to communicate directly with a service. More importantly, we continuously authenticate the user accessing the terminal, exploiting the fact that a user operating a terminal is most likely facing it most of the time. We periodically issue authentication challenges, which are displayed as a QR code on the terminal, that cause the glass device to re-authenticate the user with an appropriate response. We evaluate our system to determine the technical limits of our approach.

==> figs/Makefile <==
PLOT=pl -eps -tightcrop

TARGETS=battery.eps cpu_mem.eps qr75.eps study.eps
QRCODE_LENS=75 124 170 188 309 430 453 744 1031

all: $(TARGETS) qrcode

%.eps: %.plot Makefile
	$(PLOT) -textsize 10 -o $@ $<

qrcode: qrXXX.plot ../exps/qrcode/*.txt Makefile
	for l in $(QRCODE_LENS); do \
		sed "s/XXX/$$l/g" qrXXX.plot > qr$$l.plot ; \
		$(PLOT) -textsize 11 -o qr$$l.eps qr$$l.plot ; \
		rm qr$$l.plot ; \
	done


==> survey_table.tex <==
\begin{table}
\caption{Survey results}
\begin{center} 
      \scalebox{0.90}{ 
%%\begin{tabular}{l*{3}{l}r}
 \begin{tabular}{ | l| p{7cm} | l |}

\hline
Q2	&	General questions related to the authentication methods  & Results\\
\hline
\hline


Q2a	&	Which type of authentication method are you using in your every day life &	 \\
	&		&	\\

&	Credentials	&	100\% \\
&	Biometrics	& 	15\% 	\\
&	One-time password	&	20\%\\
&	Public Key\textbackslash Share Key	&	30\% \\
\hline
Q2b	&	How secure are the following authentication methods     \newline   (4 = very secure, 3 = secure, 2 = basic security, 1 = not secure)  & \\
	&		&	\\
&	Passwords	&	2 \\
&	Biometrics	&	2	\\
&	One-time password	&	3 \\
&	Public Key\textbackslash Share Key	&	4	\\
\hline
\hline

Q3	&	Authentication through wearable devices	&	\\
\hline\hline

Q3a	&	It's the first time you using a wearable device like Google Glass?	& \\
	&		&	\\
&	Yes	&	100\% \\
&	No	&	0\%	\\
&	No, I have already one	&	0\% \\
\hline
Q3b	&	Are you going to use wearable devices in your every day life in the close future?	& \\
	&		&	\\
&	Yes	&	0\%	\\
&	No	&	100\%	\\
&	Some of these devices	& \\
\hline
Q3c	&	Do you feel that authentication methods should be improved in the future	& \\
	&		&	\\
&	Yes	&	85\%		\\
&	No	&	15\%		\\
\hline
Q3d	&	Are able wearable devices, improve authentication process		&	\\
	&		&	\\
&	Yes, both security and usability	&	65\%		\\
&	No	&	10\%	\\
&	Yes, only usability, not security	&	25\% \\
\hline\hline
Q4	&	Improving authentication via GAuth	&	\\
\hline\hline
Q4a	&	Which of the 4 scenarios do you feel is more secure? \newline (Select only 1)	& \\
	&		&	\\
&	Credentials	&	0\% \\
&	GAuth	&	0\%	\\
&	2FA - Mobile	&	5\%	\\
&	2FA - Glass	&	0\%	\\
&	2FA - GAuth	&	95\%	\\
\hline
Q4c	&	Do you think that Google Glass can improve the authentication process	&	\\
	&		&	\\
&	Yes, both security and usability	&	20\%	\\
&	No	&	35\%	\\
&	Yes, only usability, not security	&	45\%	\\
\hline
Q4d	&	Which authentication method do you prefer? \newline (Select only 1)	&\\
	&		&	\\
&	Credentials	&	0\%	\\
&	GAuth	&	0\%	\\	
&	2FA - Mobile		&	5\%	\\
&	2FA - Glass	&	0\%	\\
&	2FA - GAuth	&	95\%	\\
\hline
Q4e & How secure are these authentication scenarios \newline  (4 = very secure, 3 = secure, 2 = basic security, 1 = not secure) & \\
	&		&	\\
&	Credentials & 2 \\
&	GAuth	&	2	\\
&	2FA - Mobile		&	3\\
&	2FA - Glass	&	3	\\
&	2FA - GAuth	&	4	\\
\hline
Q4f	&	Are you going to use GAuth in you every day life?		&	\\
	&		&	\\
&	Yes	&	75\%		\\
&	No	&	15\%		\\
\hline

\end{tabular}
}
\end{center}
\end{table}	
